An AMM minimizing user-level extractable value and loss-versus-rebalancing

We present V0LVER, an AMM protocol which solves an incentivization trilemma between users, passive liquidity providers, and block producers. V0LVER enables users and passive liquidity providers to interact without paying MEV or incurring uncontrolled loss-versus-rebalancing to the block producer. V0LVER is an AMM protocol built on an encrypted transaction mempool, where transactions are decrypted after being allocated liquidity by the AMM. V0LVER ensures this liquidity, given some external market price, is provided at that price in expectancy. This is done by incentivizing the block producer to move the pool price to the external market price. With this, users transact in expectancy at the external market price in exchange for a fee, with AMMs providing liquidity in expectancy at the external market price. Under block producer and liquidity provider competition, all of the fees in V0LVER approach zero. Without block producer arbitrage, V0LVER guarantees fall back to those of an AMM, albeit free from loss-versus-rebalancing and user-level MEV.

==> Appendices/Proofs.tex <==
\input{Appendices/RelatedWork}


==> TalkProposal.tex <==


\section{Talk Contents}
This talk is based on the the paper\cite{V0LVERMcMenamin}. In this talk, we describe $\protocolName$ \footnote{near-\textbf{0} \textbf{E}xtractable \textbf{V}alue and \textbf{L}oss-\textbf{V}ersus-\textbf{R}ebalancing $\leadsto$ \textbf{V0LVER }}, an AMM which provides arbitrarily high protection against user-level MEV and LVR. $\protocolName$ is the first AMM to align the incentives of the three, typically competing, entities in AMMs; the user, the pool, and the block producer. 
This is done by ensuring that at all times, a block producer is incentivized to move the pool to the price maximizing LVR. When the block producer chooses a price, the block producer is forced to assert this is correct, a technique introduced in \cite{DiamondMcMenamin}. Unfortunately, the protocol in \cite{DiamondMcMenamin} gives the block producer total power to extract value from users, due to order information being revealed to the block producer before it is allocated a trading price in the blockchain. To address this, $\protocolName$ is built on encrypted mempools. 

Modern cryptographic tools allow us to encrypt the mempool using zero-knowledge based collateralized commit-reveal protocols \cite{DPACCsMcMenamin,ZCash,FairTraDEXMcMenamin,TornadoCashWebsite}, delay encryption \cite{DelayEncryptionBurdges,FairPoSChiang} and/or threshold encryption \cite{HelixAsayag}. If a block producer adding an order to an AMM is forced to replicate the payoff of the AMM, we demonstrate the block producer maximizes her own utility by showing liquidity centred around the external market price.\footnote{This holds true in many CFMMs, including the famous Uniswap V2 protocol.} Providing users with an AMM where the expected trade price is the external market price, excluding fees, is a significant advancement and the main contribution of this talk. Although batching orders against AMM liquidity has been proposed as a defense against LVR \cite{BatchCFMMsRamseyer}, naively batching orders against an AMM still allows a block producer to extract LVR by censoring user orders. In $\protocolName$, block producers are effectively forced to immediately repay LVR, while always being incentivized to include order commitments in the blockchain, and eventually allocate AMM liquidity to these orders. 


